Hierarchical Attention Models for Multi-Relational Graphs

We present Bi-Level Attention-Based Relational Graph Convolutional Networks (BR-GCN), unique neural network architectures that utilize masked self-attentional layers with relational graph convolutions, to effectively operate on highly multi-relational data. BR-GCN models use bi-level attention to learn node embeddings through (1) node-level attention, and (2) relation-level attention. The node-level self-attentional layers use intra-relational graph interactions to learn relation-specific node embeddings using a weighted aggregation of neighborhood features in a sparse subgraph region. The relation-level self-attentional layers use inter-relational graph interactions to learn the final node embeddings using a weighted aggregation of relation-specific node embeddings. The BR-GCN bi-level attention mechanism extends Transformer-based multiplicative attention from the natural language processing (NLP) domain, and Graph Attention Networks (GAT)-based attention, to large-scale heterogeneous graphs (HGs). On node classification, BR-GCN outperforms baselines from 0.29% to 14.95% as a stand-alone model, and on link prediction, BR-GCN outperforms baselines from 0.02% to 7.40% as an auto-encoder model. We also conduct ablation studies to evaluate the quality of BR-GCN's relation-level attention and discuss how its learning of graph structure may be transferred to enrich other graph neural networks (GNNs). Through various experiments, we show that BR-GCN's attention mechanism is both scalable and more effective in learning compared to state-of-the-art GNNs.

==> introduction.tex <==
\section{Introduction}
\label{introduction}
Highly multi-relational data are characteristic of real-world HGs. Relational data in the HG are defined as a triple of the form \textsl{(h:head entity, r:relation, t:tail entity)}, which indicates that two entities are connected by a specific relation type. Figure~\ref{fig:movie-example} shows a HG formed by such triples (e.g., \textsl{(Movie A, actor, Celebrity Actor 1)}). Despite their usefulness, even the largest HGs such as Freebase~\cite{freebase}, DBpedia~\cite{db}, and YAGO~\cite{yago} remain incomplete and are difficult to maintain. Two fundamental HG tasks are focused on recovering incomplete knowledge, which have numerous applications including question answering (QA)~\cite{QA-as-MT-Bao, Dong-QA, hixon, seyler, QA-freebase-yao} and information retrieval~\cite{PSG, KB-kotov, pLogicN}. These are: (1) node classification, or how to infer types or categorical properties of entities based on the existing triples, and (2) link prediction, or how to recover missing triples by assigning their confidence scores using knowledge from the existing triples. 
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{fig/movie.pdf}
    \caption{\textmd{Partial sample HG of movies. The nodes are entities which belong to entity types (e.g., \textsl{person}), and the edges are relation links which belong to relation types (e.g, \textsl{actor}). The node classification task is to predict the missing entity type of the node, such as inferring the label of \textsl{2 hours} as \textsl{time}. The link prediction task is to predict the missing triple, such as \textsl{(Movie A, length, 2 hours}). (a) Neighborhood context of (a) Movie A, and (b) Movie B of one-hop neighbors.}}
    \label{fig:movie-example}
\end{figure}
Several research works have focused on proposing and improving deep neural architectures to infer missing knowledge in HGs. These include (1) GNNs, and (2) attention-based architectures. GNNs~\cite{GNNs} are deep neural networks that can effectively learn node embeddings from node features and graph structure. GNNs have been applied to various domains including social networks~\cite{Meta-GNN, social-net-graph-sage, DiffPool}, medical informatics~\cite{kidney-disease, Liver}, and software development~\cite{Verification, software-nn-survey} for representation learning. In recent years, the class of GNNs known as Graph Convolutional Networks (GCNs)~\cite{GCN}, have extended the neural network convolutional operator to graph structures. Other research works~\cite{Transformer, GAT} have advanced deep neural networks by introducing the attention mechanism, a deep learning technique that can generalize to arbitrary data to enable the neural network to focus on only the most important features of the data. Neural network attention has been applied to several domains including natural language processing (NLP)~\cite{Bert, NLP-survey, Transformer}, computer vision~\cite{cv-attention, Image-sa}, and social networks~\cite{GAT, HAN}. Despite their success, GNNs and attention-based architectures, have limitations on learning from HGs. They do not fully utilize the intra-relational interactions, or interactions between relation-specific nodes, and inter-relational interactions, or interactions between relations. As such, many critical pieces of information that can be learned from the graph, are left out entirely.  

To address the above challenges, in this paper, we present \textbf{B}i-Level Attention-Based \textbf{R}elational \textbf{G}raph \textbf{C}onvolutional \textbf{N}etworks (BR-GCN), attention-based GCNs for HGs. Our contributions are as follows. First, we present a generalized framework formulation for computing bi-level attention. Second, for each node in parallel, BR-GCN models utilize graph structural information in a sparse way by restricting the node's graph to one-hop neighbor nodes and relations. Third, our model uses a novel hierarchical attention mechanism that is inspired from Transformer-based attention and GAT-based attention. To the best of our knowledge, we are the first to extend using Transformer-based attention to HGs for GCNs. Fourth, we show how BR-GCN can be effectively used for inferring knowledge from HGs through node classification and link prediction experiments against state-of-the-art models. Using ablation studies, we also discuss how BR-GCN's learning of graph structure may be transferred to enrich other GNNs. As suggested by strong empirical evidence, our technique powerfully leverages bi-level attention and GCNs to scalably capture both intra-relational and inter-relational interactions in HGs for better representation learning. 

The remainder of this paper is organized as follows. In Section~\ref{related-work}, we examine the related work. Section~\ref{BR-GCN-architecture} presents a generalized formulation for the bi-level attention used by BR-GCN, and describes BR-GCN's architecture. Section~\ref{evaluation} presents experimental results of BR-GCN in comparison to state-of-the-art models for node classification, link prediction, and ablation studies. Section~\ref{conclusions} concludes. 


==> related_work.tex <==
\section{Related Work}
\label{related-work}

\subsection{Attention-Based Neural Networks}
Multiplicative and additive attention are state-of-the-art attention mechanisms used in neural networks~\cite{ neural-mt, sen-sum, end-end, Transformer, GAT}. Multiplicative attention is computed using an inner product or cosine similarity of encoder states. Additive attention is computed through a linear combination or concatenation of encoder states. Transformer and GAT are leading-edge attention-based neural architectures.

\paragraph{Transformer}
Transformers~\cite{Transformer} are attention-based models specific to NLP, which have been utilized for machine translation tasks~\cite{Transformer-mt, universal-transformer, Transformer}, and more recently, QA~\cite{trans-qa, transformer-xh}, sentence completion~\cite{T-CVAE}, and sentiment analysis~\cite{Transformer-sentiment, Transformer-sentiment2}. Through multiplicative attention, Transformer captures the feature similarity over all tokens $j$ for token $i$ in the sequence, which is used to weight token $j$ for learning $i$'s embedding. However, as Transformer's attention for each token in the sequence requires operations on all other tokens in the sequence, it is not feasible for large-scale input.

\paragraph{Graph Attention Networks:} 
GAT~\cite{GAT} are additive attention-based GNNs that address the limitations of Transformer's scalability by effectively leveraging graph structure and sparsity to compute a node's attention. In HGs, as different nodes play different roles, attention is required at the node-level to distinguish these nodes by importance. GAT models, however, are limited to homogeneous graphs, or graphs that only include one type of node or relation, eventhough HGs contain different relations that may have different levels of importance for a node. 

\subsection{Relational Graph Convolutional Networks}
R-GCN architectures~\cite{rgcn} extend GCNs and GAT, which operate on local graph neighborhoods of homogeneous graphs, to operate on multi-relational graphs by distinguishing nodes by relation type. R-GCN models, however, treat all relation-specific nodes as equally important. Further, R-GCN models do not utilize graph attention as they are limited to directly learning from weight parameters.


\subsection{Heterogeneous Graph Attention Networks}
To address the limitations of the above models, Heterogeneous Graph Attention Networks (HAN)~\cite{HAN} integrate bi-level attention with GNNs to learn node embeddings. HAN's bi-level attention mechanism learns both node-level attention and relation-level attention. HAN models, however, have limitations. First, they learn relation-level attention for a node based on how similar each neighborhood relation is to a global learnable weight vector. Relational comparison to a global vector treats relations as independent from each other due to lack of direct local inter-relation comparison, and as so, does not learn relation-level attention that is personalized to each node. Second, HAN models only consider the heterogeneous subgraph contained by pre-defined meta-paths, which are computationally expensive to compute and may also be sub-optimal in identifying salient graph components.  
\begin{table*}[t!]
  \caption{\textmd{Variables (Var) and Explanations. Table on the left column corresponds to node-level attention. Table on the right column corresponds to relation-level attention.}}
  \label{tab:dataset_description}
  \centering
  \begin{tabular}{cc|cc}
  \hline
Var & Explanation & Var & Explanation \\ [0.5 ex]
\hline
$r$ & Relation on node edge & $\textbf{W}_{1, r}$ & Projection weight matrix for $z_{i}^{r}$\\[0.5ex]
$R_{i}$ & Set of relations on edge of node $i$ & $\textbf{W}_{2, r}$ & Projection weight matrix for $z_{i}^{r}$\\[0.5ex] 
$\textbf{h}_{i}^{(l)}$ & Node $i$ features at layer $l$ & $\textbf{W}_{3, r}$ & Projection weight matrix for $z_{i}^{r}$\\[0.5ex]
$e_{i,j}^{r}$ & GAT-based attention for $(i,j)$ & $\textbf{q}_{r, i} \in Q_{r}$  & Transformer-based query matrix row\\[0.5ex]
$\mathrm{edge}_{i, j}$ & Edge between node $i$ and node $j$ & $\textbf{k}_{r, i} \in K_{r}$ & Transformer-based key matrix row\\[0.5ex]
$\textbf{a}_{r}$ & Relation-specific attention vector & $\textbf{v}_{r, i} \in V_{r}$ & Transformer-based value matrix row\\[0.5ex]
$\gamma_{i,j}^{r}$ & Relation-specific weight for $(i,j)$ & $\textbf{W}_{i}$ & Weight matrix for $h_{i}^{(l)}$\\[0.5ex]
$N_{i}^{r}$ &  Set of relation-specific node neighbors & $\psi_{i}^{r}$ & Importance of relation $r$ for node $i$\\[0.5ex]
$\textbf{z}_{i}^{r}$ &  Relation-specific node embedding & $\boldsymbol{\delta}_{i}^{r}$ & Attended relation-specific embedding\\[0.5ex]
\arrayrulecolor{black}\hline
 \end{tabular}
\end{table*}






==> tables/data-stats-split.tex <==
\begin{table}
\centering
\caption{\textmd{\small{
  Dataset statistics for entities $E$, concepts $C$ and their relations. $E-E$ denotes entity-entity links, $C-C$ denotes concept-concept links, and $E$-$C$ denotes entity-concept links.}}}
 \vspace{-2mm}
{
\footnotesize
\begin{tabular}{c|cc|ccc}
\bottomrule
Dataset &
\multicolumn{2}{c|}{Nodes} &
\multicolumn{3}{c}{Relations} \\
  & \#$E$ & \#$C$ & \#$E$-$E$: $R_{I}$ & \#$C$-$C$: $R_{O}$ & \#$E$-$C$: $R_{IO}$\\
\hline
 YAGO26K-906 & 26,078 & 906 &  390,738 &  8,962 & 9,962 \\
 DB111K-174 & 111,762 & 174 & 863,643 &  763 & 99,748 \\
 \toprule
\end{tabular}
\vspace{-2mm}
}
\label{tab:dataset-stat}
\end{table}

\vspace{-2mm}
\begin{table}
\centering
\caption{\textmd{\small{
  Data splits for triple completion and entity typing. We provide splits for all KG triples in $R_{I}, R_{O}, R_{IO}$ for train(tr), validation(v), and test(ts).}}}
\vspace{-2mm}
{
\footnotesize
\begin{tabular}{c|ccc}
\bottomrule
 & &
 YAGO26K-906 &  \\
Task &
Tr($R_{I}/R_{O}/R_{IO}$) & V($R_{I}/R_{O}/R_{IO}$) & Ts($R_{I}/R_{O}/R_{IO}$) \\
\hline
Triple Completion & 332,128/7,618/8,691 & 19,536/448/485 & 39,074/896/1,019\\
Entity Typing & 211,346/4,876/5,379 & 23,549/543/598 & 156,311/3,592/3,985\\
\hline
\hline
 & &
 DB111K-174 &  \\
Task &
Tr($R_{I}/R_{O}/R_{IO}$) & V($R_{I}/R_{O}/R_{IO}$) & Ts($R_{I}/R_{O}/R_{IO}$) \\
\hline
Triple Completion & 734,096/648/84,864 & 43,182/38/5,018 & 86,365/77/10,131 \\
Entity Typing & 466,538/462/53,863 & 51,828/46/5,985 & 345,504/337/39,900 \\
\toprule
\end{tabular}
}
\label{tab:data-split}
\vspace{-1mm}
\end{table}

==> tables/table-entity-type.tex <==
\begin{table}
\caption{\textmd{\small{
  Results of entity typing. For each group of models, the best results are bold-faced. The overall best results on each dataset are underscored.}}}
\vspace{-2mm}
\footnotesize
%\resizebox{\linewidth}{!}{
\setlength\tabcolsep{2.5pt}
{
\begin{tabular}{c|ccc|ccc}
\bottomrule
{Datasets} &
\multicolumn{3}{c|}{YAGO26K-906} &
\multicolumn{3}{c}{DB111K-174}
\\
% Row 2
{Metrics} & 
MRR & Acc. & Hit@3 &
MRR & Acc. & Hit@3
\\
\hline
\hline
% Row 3-4 Baselines
{\transe} 	& 0.144 & 7.32 	& 35.26	& 0.503 & 43.67 & 60.78\\
{\distmult} 	& 0.411 & 36.07 & 55.32 & 0.551 & 49.83 & 68.01\\ 
{\complex} 	& 0.519 & 43.08 & 59.28 & 0.583 & 55.07 & 70.17\\ 
{\rotate} 	& 0.673 & 58.24 & 73.95 & 0.721 & 61.48 & 75.67\\
{\joie} 	& 0.899 & 85.72 & 96.02 & 0.859 & 75.58 & 96.02\\ 
{\hyperkg} 	& 0.627 & 55.39 & 65.64 & 0.736 & 61.20 & 74.29\\ 
{\hake} 	& 0.905 & 87.42 & 96.37 & 0.866 & 76.04 & 96.22\\ 
{\cone} 	& \textbf{0.912} & \textbf{87.51} & \textbf{96.39} & \textbf{0.869} & \textbf{76.85} & \textbf{96.38}\\ 
\hline
{\rehf} 	& 0.907 & 87.49 & 96.37 & 0.867 & 76.26 & 96.31\\ 
{\roth} 	& 0.909 & 87.49 & 96.39 & 0.868 & 76.55 & 96.36\\ 
{\atth} 	& 0.910 & 87.50 & 96.38 & 0.868 & 76.50 & 96.33\\ 
{\hgcn} 	& 0.905 & 87.44 & 96.37 & 0.867 & 76.11 & 96.27\\ 
{\hyperka} 	& 0.918 & 87.76 & 96.45 & 0.871 & 76.65 & 96.50\\ 
{\mtwognn} 	& \textbf{0.922} & \textbf{88.16} & \textbf{97.01} & \textbf{0.880} & \textbf{77.58} & \textbf{96.94}\\ 
\hline
\rowcolor{shadecolor} {\ourmodel ($\mathbb{S}^{d}/\mathbb{S}^{d}$)} 	& 0.919 & 87.94 & 96.81 & 0.875 & 77.03 & 96.78\\ 
\rowcolor{shadecolor} {\ourmodel ($\mathbb{H}^{d}/\mathbb{H}^{d}$)} 	& \textbf{0.924} & \textbf{88.12} & \textbf{97.01} & \textbf{0.887} & \textbf{77.53} & \textbf{96.95}\\ 
\rowcolor{shadecolor} {\ourmodel ($\mathbb{E}^{d}/\mathbb{H}^{d}$)} 	& 0.922 & 88.07 & 96.91 & 0.883 & 77.37 & 96.58\\ 
\rowcolor{shadecolor} {\ourmodel ($\mathbb{S}^{d}/\mathbb{E}^{d}$)} 	& 0.917 & 87.68 & 96.41 & 0.866 & 76.33 & 96.48\\ 
\hline
\rowcolor{shadecolor} {\ourmodel-RO-FC} 	& 0.930 & 88.47 & 97.32 & 0.891 & 77.81 & 97.04\\ 
\rowcolor{shadecolor} {\ourmodel-SO-FC} 	& 0.938 & 89.02 & 98.11 & \underline{\textbf{0.895}} & 77.92 & 97.40\\ 
\rowcolor{shadecolor} {\ourmodel (ours)} 	& \underline{\textbf{0.939}} & \underline{\textbf{89.07}} & \underline{\textbf{98.18}} & \underline{\textbf{0.895}} & \underline{\textbf{77.94}} & \underline{\textbf{97.47}}\\ 
\toprule
\end{tabular}
}
\label{tab:type}
\end{table}

==> tables/table-kg-compl.tex <==
\begin{table*}[!htb]
\caption{\textmd{\small{
  Results of KG triple completion. $\boldsymbol{M}$ denotes the $d$-dimensional manifold space, $R_{I}$ are entity links, $R_{O}$ are concept links. For each group of models, the best results are bold-faced. The overall best results on each dataset are underscored.}}}
 \vspace{-2mm}
\centering
{
\footnotesize
\begin{tabular}{c|c|c|ccc|ccc||ccc|ccc}
\bottomrule
 & & {Datasets} &
\multicolumn{6}{c||}{YAGO26K-906} &
\multicolumn{6}{c}{DB111K-174}
\\
% \hline
% Row 2
Type & $\boldsymbol{M}$ & {Graphs} &
\multicolumn{3}{c}{$R_I$ KG Completion} &
\multicolumn{3}{c||}{$R_O$ KG Completion} & 
\multicolumn{3}{c}{$R_I$ KG Completion} &
\multicolumn{3}{c}{$R_O$ KG Completion}
\\
% \hline
% Row 3
& & {Metrics} & 
MRR & H@1 & H@10 &
MRR & H@1 & H@10 &
MRR & H@1 & H@10 &
MRR & H@1 & H@10 
\\
\hline
\hline
% Row 4-6 Baselines
& $\mathbb{E}^{d}$ & {\transe} & 0.187 & 13.73 & 35.05 & 0.189 & {14.72} & 24.36 & 0.318 & 22.70 & 48.12 & 0.539 & 47.90 & 61.84 \\
& $\mathbb{E}^{d}$ & {\distmult} & 0.288 & 24.06 & 31.24 & 0.156 & 14.32 & 16.54 & 0.280 & 27.24 & 29.70 & 0.501 & 45.52 & 64.73\\
 non-GNN based& $\mathbb{C}^{d}$ & \complex & 0.291 & 24.85 & 37.28 & 0.180 & 14.83 & 22.97 & 0.321 & 27.39 & 46.63 & 0.549 & 47.80 & 62.23 \\
KGE models & $\mathbb{C}^{d}$ & {\rotate} & 0.302 & \textbf{25.31} & 42.17 & 0.228 & 16.35 & 27.28 & 0.356 & 29.31 & 54.60 & 0.557 & 49.16 & 68.19 \\
& $\mathbb{E}^{d}$ & {\joie} & \textbf{0.316} & 24.62 & \textbf{51.85} & 0.289 & 18.66 & 39.13 & \textbf{0.479} & \textbf{35.21} & \textbf{72.38} & 0.602 & 52.48 & 79.71 \\
& $\mathbb{H}^{d}$ & {\hyperkg} & 0.215 & 18.35 & 36.02 & 0.174 & 14.50 & 23.26 & 0.302 & 23.31 & 46.72 & 0.542 & 47.59 & 62.11 \\
& $\mathbb{H}^{d}$ & {\hake} & 0.293 & 23.04 & 40.19 & 0.301 & 19.27 & 41.09 & 0.391 & 31.10 & 60.46 & 0.638 & 55.69 & 81.07 \\
& $\mathbb{H}^{d}$ & {\cone} & 0.299 & 23.56 & 41.23 & \textbf{0.313} & \textbf{20.05} & \textbf{41.80} & 0.422 & 33.69 & 68.12 & \textbf{0.639} & \textbf{55.89} & \textbf{81.45} \\
\hline
& $\mathbb{H}^{d}$ & {\rehf} & 0.282 & 23.19 & 40.52 & 0.298 & 19.70 & 41.26 & 0.407 & 30.06 & 66.93 & 0.622 & 55.35 & 81.09 \\
& $\mathbb{H}^{d}$ & {\roth} & 0.295 & 23.50 & 41.03 & 0.308 & 19.97 & \textbf{41.78} & 0.418 & 30.18 & 67.05 & 0.639 & 55.82 & 81.44 \\
GNN-based models& $\mathbb{H}^{d}$ & {\atth} & 0.298 & 23.43 & 41.20 & 0.310 & 19.99 & 41.53 & 0.419 & 30.10 & 66.58 & 0.629 & 55.37 & 81.39 \\
& $\mathbb{H}^{d}$ & {\hgcn} & 0.307 & 23.04 & 40.25 & 0.302 & 19.38 & 40.49 & 0.396 & 31.54 & 61.78 & 0.638 & 55.81 & 81.60 \\
& $\mathbb{H}^{d}$ & {\hyperka} & 0.320 & 26.71 & 52.09 & 0.305 & 18.83 & 40.28 & 0.486 & 35.79 & 72.33 & 0.613 & 53.36 & 80.59 \\
& $\mathbb{P}^{d}$ & {\mtwognn} & \textbf{0.347} & \textbf{29.63} & \textbf{54.28} & \textbf{0.341} & \textbf{23.70} & 42.19 & \textbf{0.506} & \textbf{36.52} & \textbf{73.11} & \textbf{0.644} & \textbf{56.82} & \textbf{83.01} \\
\hline
\rowcolor{shadecolor} & -- & \ourmodel ($\mathbb{S}^{d}/\mathbb{S}^{d}$) & \textbf{0.338} & \textbf{27.15} & \textbf{53.20} & 0.318 & 20.36 & 41.02 & 0.491 & 34.58 & 71.40 & 0.606 & 53.29 & 80.17\\
\rowcolor{shadecolor} Ablation variants: & -- & \ourmodel ($\mathbb{H}^{d}/\mathbb{H}^{d}$) & 0.314 & 25.11 & 52.02 & \textbf{0.358} & \textbf{24.61} & \textbf{43.28} & \textbf{0.502} & \textbf{35.79} & \textbf{73.61} & \textbf{0.663} & \textbf{57.59} & \textbf{84.16}\\
\rowcolor{shadecolor} \ourmodel ($R_{I}/R_{O}$) & -- & \ourmodel ($\mathbb{E}^{d}/\mathbb{H}^{d}$) & 0.327 & 25.32 & 52.89 & 0.343 & 23.95 & 41.62 & 0.498 & 35.11 & 72.37 & 0.640 & 56.17 & 82.68\\
\rowcolor{shadecolor} & -- & \ourmodel ($\mathbb{S}^{d}/\mathbb{E}^{d}$) & 0.322 & 24.91 & 52.36 & 0.297 & 19.43 & 40.61 & 0.484 & 33.29 & 73.54 & 0.619 & 53.72 & 80.51\\
\hline
\rowcolor{shadecolor} & -- & {\ourmodel-RO-FC} & 0.352 & 29.79 & 55.21 & 0.364 & 25.04 & 43.27 & 0.518 & 37.65 & 73.97 & 0.681 & 59.23 & 84.16\\
\rowcolor{shadecolor} \ourmodel variants & -- & {\ourmodel-SO-FC} & 0.364 & \underline{\textbf{30.15}} & 55.93 & 0.369 & 25.81 & 44.18 & \underline{\textbf{0.536}} & 38.29 & 74.28 & 0.687 & 59.26 & \underline{\textbf{84.82}}\\
\rowcolor{shadecolor} & -- & \ourmodel (ours) & \underline{\textbf{0.366}} & \underline{\textbf{30.15}} & \underline{\textbf{56.06}} & \underline{\textbf{0.372}} & \underline{\textbf{25.88}} & \underline{\textbf{44.38}} & \underline{\textbf{0.536}} & \underline{\textbf{38.31}} & \underline{\textbf{74.85}} & \underline{\textbf{0.690}} & \underline{\textbf{59.88}} & \underline{\textbf{84.82}}\\
\toprule
\end{tabular}
\vspace{-3mm}
}
\label{tab:link}

\end{table*}
